Simulation of Spin Chains with off-diagonal Coupling Using Inchworm Method

We study the dynamical simulation of open quantum spin chain with nearest neighboring coupling, where each spin in the chain is associated with a harmonic bath. This is an extension of our previous work [G. Wang and Z. Cai, J. Chem. Theory Comput., 19, 8523--8540, 2023] by generalizing the application of the inchworm method and the technique of modular path integrals from diagonally coupled cases to off-diagonally coupled cases. Additionally, to reduce computational and memory cost in long time simulation, we apply tensor-train representation to efficiently represent the reduced density matrix of the spin chains, and employ the transfer tensor method (TTM) to avoid exponential growth of computational cost with respect to time. Abundant numerical experiments are performed to validate our method.

==> Path_Integral/Path_Integral.tex <==
% \section{Diagrammatic Representation of the Path Integral}
\section{Spin chain decouple}
\label{sec_diagrammatic_representation}
% \zc{change section title: If we use "Diagrammatic", then mention previous literature that uses diagrams to represent path integrals; otherwise, since we have only 1 diagram in this section, we can change the title.}
% \ki{I changed the section title but not sure about whether it is a good choice.}
In the following analysis,
 we split the total Hamiltonian $H$ into the following two parts:
\begin{equation}
\begin{split}
&H_0 \coloneqq \sum_{k=1}^K H_0^{(k)}:=\sum_{k=1}^K\left(H_s^{(k)}+H_b^{(k)}+W_s^{(k)} \otimes W_b^{(k)}\right),  \\
&V \coloneqq \sum_{k=1}^{K-1} V^{(k,k+1)}
\end{split}
\end{equation}
Below, we will assume that the interaction between spins $V$ is a perturbation of the unperturbed Hamiltonian $H_0$, and describe the dynamics in the interaction picture.

To describe the dynamics within the interaction picture, we revisit the integral form of the Liouville-von Neumann equation  \cite{breuer2002theory}:
\begin{equation}\label{eq:liouv_int}
    \rho_I(t)=\rho_I(0)-\mathrm{i} \int_0^t\left[V_I\left(s_1\right), \rho_I\left(s_1\right)\right] \mathrm{d} s_1
\end{equation}
where $\rho_I(t)=\e^{\ii  H_0 t}\e^{-\ii  H t}\rho(0)\e^{\ii  H t}\e^{-\ii H_0 t}$ denotes the density matrix in the interaction picture, and $V_I(t)= \e^{\ii H_0 t}V \e^{-\ii H_0 t}$ is the interaction picture representation of the coupling operator.
Iteratively integrating this equation,  we can expand $\rho_I(t)$ into the following Dyson series

\begin{equation}\label{eq:rhoi_dyson}
    \rho_I(t)=\sum_{N=0}^{\infty}(-\mathrm{i})^N \int_{-t \leqslant s \leqslant t}\left(\prod_{n=1}^N  \operatorname{sgn}\left(s_n\right)\right) \mathcal{T}\left[V_I\left(s_N\right) \cdots V_I\left(s_1\right) \rho_I(0)\right] \mathrm{d} \boldsymbol{s}
\end{equation}
% where $\mathcal{T}$ represents the time-ordering operator that sorts the operators in descending order. Specifically, for any time-dependent operator $A(t)$, we have
% \begin{equation}
%     \mathcal{T}[A(t_N)\cdots A(t_1)]=A(t_{i_N})\cdots A(t_{i_1}),\quad \text{where}\quad t_{i_1}\leqslant \dots\leqslant t_{i_N}.
% \end{equation}
% \yx{definition by permutation:
% where $\mathcal{T}$ represents the time-ordering operator that sorts the operator in descending order. Specifically, for a product of $N$ operators $A(t_1)\ldots A(t_N)$,
% $$\mathcal{T}\left[A(t_1)\ldots A(t_n)\right]=\sum_{\pi}\theta\left[t_{\pi(1)}-t_{\pi(2)}\right]\ldots \theta\left[t_{\pi(N-1)}-t_{\pi(N)}\right]A(t_{\pi(1)})\ldots A(t_{\pi(N)})$$
% where $\theta(x)$ is the Heasviside step function and $\pi$ is a permutation of $N$ indexes and the sum extends over all $N!$ different permutations.
% }
where $\mathcal{T}$ represents the time-ordering operator that sorts the operators in descending order.
Specifically, for the product of $N$ operators, $A(t_1),\dots,A(t_N)$,
\begin{equation}
    \mathcal{T}[A(t_N)\dots A(t_1)]
    = A(t_{\pi(N)}) \dots A(t_{\pi(1)})
\end{equation}
with $\pi$ being the permutation satisfying
\begin{equation}
    t_{\pi(1)} \leqslant t_{\pi(2)} \leqslant \dots \leqslant t_{\pi(N)}.
\end{equation}
% Specifically, for a product of $N$ operators $A(t_1)\ldots A(t_N)$,
% $$\mathcal{T}\left[A(t_1)\ldots A(t_n)\right]=\sum_{\pi}\theta\left[t_{\pi(1)}-t_{\pi(2)}\right]\ldots \theta\left[t_{\pi(N-1)}-t_{\pi(N)}\right]A(t_{\pi(1)})\ldots A(t_{\pi(N)})$$
% where $\theta(x)$ is the Heasviside step function and $\pi$ is a permutation of $N$ indexes and the sum extends over all $N!$ different permutations.
% \ki{
%     Specifically, for the product of $N$ operators, $A(t_1),\dots,A(t_N)$,
% \begin{equation}
%     \mathcal{T}[A(t_N)\dots A(t_1)]
%     = A(t_{\pi(N)}) \dots A(t_{\pi(1)})
% \end{equation}
% with $\pi$ being the permutation satisfying
% \begin{equation}
%     \pi(1) \leqslant \pi(2) \leqslant \dots \leqslant \pi(N).
% \end{equation}
% }
The full form of the integral in (\ref{eq:rhoi_dyson}) is 
\begin{equation}
    \int_{-t\leqslant \boldsymbol{s}\leqslant t} 
    \text{(integrand)}
    \dd\boldsymbol{s}
    = \int_{-t}^{t} 
    \int_{-t}^{s_N}
    \dots
    \int_{-t}^{s_2}
    \text{(integrand)}
    \dd s_1 
    \dots
    \dd s_{N-1}
    \dd s_N
\end{equation}
where the domain is an $N$-dimensional simplex.
We can also represent \cref{eq:rhoi_dyson} by the following diagrammatic form
\begin{equation*}
    \rho_I(t)
    = \begin{tikzpicture}[baseline=0]
    \filldraw[fill=black] (-1,-0.1) rectangle (1,0.1);
    \node[text=black,anchor=north] at (-1,0) {$-t$};
    \node[text=black,anchor=north] at (1,0) {$t$};
    \end{tikzpicture}
    +   
    \begin{tikzpicture}[baseline=0]
    \filldraw[fill=black] (-1,-0.1) rectangle (1,0.1);
    \node[text=black,anchor=north] at (-1,0) {$-t$};
    \node[text=black,anchor=north] at (1,0) {$t$};
    %\node[text=red] at (-0.5,0) {$\times$};
    \draw plot[only marks, mark=x, mark options={color=applegreen, scale=2, ultra thick}] coordinates {(-0.5,0)};
    \node[text=black,anchor=north] at (-0.5,0) {$s_1$};
    \end{tikzpicture}
    + 
    \begin{tikzpicture}[baseline=0]
    \filldraw[fill=black] (-1,-0.1) rectangle (1,0.1);
    \node[text=black,anchor=north] at (-1,0) {$-t$};
    \node[text=black,anchor=north] at (1,0) {$t$};
    \draw plot[only marks, mark=x, mark options={color=applegreen, scale=2, ultra thick}] coordinates {(-0.5,0)};
    \node[text=black,anchor=north] at (-0.5,0) {$s_1$};
    \draw plot[only marks, mark=x, mark options={color=applegreen, scale=2, ultra thick}] coordinates {(0.3,0)};
    \node[text=black,anchor=north] at (-0.5,0) {$s_1$};
    \node[text=black,anchor=north] at (0.3,0) {$s_2$};
    \end{tikzpicture}
    + \dots
\end{equation*}
where the first diagram corresponding to the term in \cref{eq:rhoi_dyson} with $N=0$.
In the second diagram, there is a green cross at $s_1$, representing the term with $N=1$ in \cref{eq:rhoi_dyson}.
In the third diagram, we have two crosses standing for the two interaction operators $V_I(s_1)$ and $V_I(s_2)$.
Within this framework, we generalize the expression of coupling operator $V_I(s_n)$ to:
\begin{equation}\label{op:v_i}
\begin{split}
    V_I\left(s_n\right)
    \coloneqq & \mathrm{e}^{\mathrm{i} H_0\left|s_n\right|} V \mathrm{e}^{-\mathrm{i} H_0\left|s_n\right|} \\
    = & \sum_{k=1}^{K-1}\sum_{\alpha_k\in A}V_{I,\alpha_k}^{(k)}(s_n)\otimes V_{I,\alpha_k}^{(k+1)}(s_n)
\end{split}
\end{equation}
where
\begin{equation}\label{op:v_i_k}
    V_{I,\alpha_k}^{(k)}(s_n):=\mathrm{e}^{\mathrm{i} H_0^{(k)}\left|s_n\right|}V_{\alpha_k}^{(k)}\mathrm{e}^{-\mathrm{i} H_0^{(k)}\left|s_n\right|}
\end{equation}

By assuming the initial density matrix is separable, i.e., $\rho(0) = \bigotimes_{k=1}^K \rho^{(k)}(0)$, we can decouple $\rho_{I}(t)$ among spins,
\yx{$\boldsymbol{s}^k$}
\begin{equation}
\label{eq_rho_k}
\begin{gathered}
    \rho^{(k)}(\boldsymbol{s}',\boldsymbol{\alpha}_k')
    = \left(\prod_{n'=1}^{N'} \sqrt{-\ii\,\sgn(s_{n'}')} \right)
    \mathcal{T}\left[
    V_{{I,\alpha_{k}^{(N')}}}^{(k)}(s_{N'}') \dots V_{I,\alpha_{k}^{(1)}}^{(k)}(s_1') \rho^{(k)}(0)
    \right]\\
    \boldsymbol{\alpha}_{k}'
    = \left(
        \alpha_k^{(1)}, \dots, \alpha_k^{(N')}
    \right) \in A^{N'}
\end{gathered}
\end{equation}

where $\boldsymbol{s}'$ is a subsequence of $\boldsymbol{s}$ of length $N' \leqslant N$. 
The sequence $\boldsymbol{\alpha}_{k}'$ has the same length as $\boldsymbol{s}'$, with each element $\alpha_k^{(j)}\in A$ having $|A|$ possible choices, representing the types of 
Here, we use $\vert A \vert$ to denote the cardinality of set $A$.
In particular, if $\boldsymbol{s'}$ is an empty sequence, we use the notation $\rho^{(k)}(\varnothing)\coloneqq \rho_{I}^{(k)}(0)$ to denote the above quantity. 
We illustrate the separability of these propagators by showing an example of $N=1$ and $K=4$, the corresponding summand in (\ref{eq:rhoi_dyson}) has has the form:

\begin{equation} \label{eq:rhoi_n1_k4}
\begin{split}
    &\int_{-t}^t
    -\ii \, \sgn(s_1)
    \mathcal{T}\left[V_I(s_1)\rho_{I}(0)\right]
    \dd s_1 \\
    =&\sum_{\alpha_{1}^{(1)}\in A^1}\int_{-t}^t \rho^{(1)}(s_1,\alpha_1^{(1)})
     \otimes \rho^{(1)}(s_1,\alpha_1^{(1)})
     \otimes \rho^{(3)}(\varnothing)
     \otimes \rho^{(4)}(\varnothing) \dd s_1\\
     +&\sum_{\alpha_2^{(1)}\in A^1}\int_{-t}^t \rho^{(1)}(\varnothing)
     \otimes \rho^{(2)}(s_1,\alpha_2^{(1)})
     \otimes \rho^{(3)}(s_1,\alpha_2^{(1)})
     \otimes \rho^{(4)}(\varnothing) \dd s_1\\
    +&\sum_{\alpha_3^{(1)}\in A^1}\int_{-t}^t \rho^{(1)}(\varnothing)\otimes\rho^{(2)}(\varnothing)
     \otimes \rho^{(3)}(s_1,\alpha_3^{(1)})
     \otimes \rho^{(4)}(s_1,\alpha_3^{(1)}) \dd s_1
\end{split}
\end{equation}


We shall use the diagrammatic equations to denote the path integrals as introduced in the previous research \cite{wang2023real} for brevity. 
Consider the scenario where the coupling operators acting on neighboring spins have three distinct types $A=\{a_1,a_2,a_3\}$.
In a four-spin chain, the first term in \cref{eq:rhoi_dyson} can be simply represented by the following diagrammatic equation. 
% \ki{I changed the color here. Would you please also change the colors in \cref{diagram_model} and \cref{P2}?} \yx{okay!!}
\input{Path_Integral/diagram_equation}%
In the diagrammatic equation above, the solid bold line on the left-hand side represents an operator of all possible types acting on all spins.
The first equality means that the inter-spin interaction can occur in any two neighboring spins and each gray line stands for a spin.
For the second equality, the crosses with three different colors on the right-hand side denote the coupling operators of different types, $a_1$, $a_2$ and $a_3$. The two gray lines connected by colored crosses represent the two spins involved in the corresponding coupling. Since there are four spins and one time point $s_1$, each cross can have three possible locations, with each location permitting three choices of coupling types. Consequently, there are $(3\times3)^1$ diagrams on the right-hand side. 
For the second term in \cref{eq:rhoi_dyson},
 we may also employ the same idea so that it would be written as the sum of 81 diagrams.

In general, for a chain with $K$ spins, the $N$th term in \cref{eq:rhoi_dyson} can be written as the sum of $\vert A \vert^N (K-1)^N$ diagrams.
In other words, \cref{eq:rhoi_dyson} can be written as the sum of diagrams, and for each diagram, the spin-chain problem is decoupled into the problems on each spin.
For a chain with $K$ spins, we in principle should consider a problem on a $2^K$-dimensional space.
With this process, we may instead consider many problems in the space of a single spin, a $2$-dimensional space.
In particular, Wang and Cai's work \cite{wang2023real} can be regarded as a special case where $\vert A \vert = 1$.

In practice, it would be impossible to sum up all the diagrams until infinity.
Since we can now decompose the original problem into problems on a single spin,
we introduce a truncation parameter $\bar{N}$ for the maximum number of interactions on each spin and its neighbor spins so that each gray line in \cref{eq_diagrammatic_expansion} would have at most $\bar{N}$ crosses in total.

So far, we have decoupled the total density matrix in the interaction picture, $\rho_I(t)$, into a sum of spin-specific 
density-matrix-like quantities $\rho^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_k)$, 
which exhibit similar structures and are independently characterized for each spin, as indicated by (\ref{eq:rhoi_dyson}). 
The Hamiltonian in (\ref{op:v_i_k}) has the form $H_0^{(k)}=H_s^{(k)} + H_b^{(k)} + W_s^{(k)} \otimes W_b^{(k)}$. Given our focus on the dynamics of the reduced density matrix $\rho_{I,s}(t) \equiv \operatorname{tr}_b\{\rho_I(t)\}$, we apply Dyson series expansion again on $H_0^{(k)}$
to separate the system-bath components within each $\rho^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_k)$, 

\begin{equation}\label{eq:rhoi_k_dyson}
    \begin{split}
        \rho^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_k)
    = &\left(\prod_{n=1}^{N} \sqrt{-\ii\,\sgn(s_{n})} \right)\sum_{M=0}^{\infty} (-\mathrm{i})^M\int_{-t\leqslant \boldsymbol{\tau}\leqslant t}\left(\prod_{m=1}^M  \operatorname{sgn}\left(\tau_m\right)\right)\\
    &\times \mathcal{U}_0^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_{k},\boldsymbol{\tau}) \otimes \mathcal{T}\left[W_{b,I}^{(k)}(\tau_1)\ldots W_{b,I}^{(k)}(\tau_M)\rho_b^{(k)}(0)\right] \mathrm{d} \boldsymbol{\tau}
    \end{split}
\end{equation}
where $\boldsymbol{\tau} = (\tau_1,\dots,\tau_M)$ is an ascending time sequence and
\begin{equation}
    \mathcal{U}_0^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau})=\mathcal{T}\left[V_{s,I, \alpha_k^{(1)}}^{(k)}\left(s_1\right) \ldots V_{s, I,\alpha_k^{(N)}}^{(k)}\left(s_N\right) W_{s, I}^{(k)}\left(\tau_1\right) \ldots W_{s, I}^{(k)}\left(\tau_M\right) \rho_{s}^{(k)}(0)\right]
\end{equation}
with
\begin{align}
    V_{s, I,\alpha_k^{(n)}}^{(k)}(s)&=\mathrm{e}^{\mathrm{i} H_{s}^{(k)}|s_n|} V_{\alpha_k}^{(k)} \mathrm{e}^{-\mathrm{i} H_s^{(k)}|s_n|}\\
    W_{s, I}^{(k)}(\tau)&=\mathrm{e}^{\mathrm{i} H_s^{(k)}|\tau|} W_s^{(k)} \mathrm{e}^{-\mathrm{i} H_s^{(k)}|\tau|}\\
    W_{b,I}^{(k)}(\tau)&=\e^{\ii H_b |\tau|}W_b^{(k)} \mathrm{e}^{-\mathrm{i} H_b^{(k)}|\tau|}
\end{align}

After tracing out the bath components, we obtain the reduced density matrix in the interaction picture represented by the Dyson series:
\begin{equation}\label{eq:rhos_dyson}
    \begin{split}
    \rho_{s,I}^{(k)}\left(\boldsymbol{s},\boldsymbol{\alpha}_k\right)
    = &\left(\prod_{n=1}^{N} \sqrt{-\ii\,\sgn(s_{n})} \right)\sum_{M=0}^{\infty} (-\mathrm{i})^M \int_{-t \leqslant \boldsymbol{\tau} \leqslant t}\left(\prod_{m=1}^M \operatorname{sgn}\left(\tau_m\right)\right) \\
    & \times \mathcal{U}_0^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_{k},\boldsymbol{\tau}) \mathcal{L}_b^{(k)}(\boldsymbol{\tau}) \mathrm{d} \boldsymbol{\tau}
    \end{split}
\end{equation}
where $\mathcal{L}_b^{(k)}(\boldsymbol{\tau})$ is the bath influence functional, defined as
\begin{equation}
    \mathcal{L}_b^{(k)}(\boldsymbol{\tau})=\operatorname{tr}_b \left\{\mathcal{T}\left[W_{b,I}^{(k)}(\tau_1)\ldots W_{b,I}^{(k)}(\tau_M)\rho_b^{(k)}(0)\right]\right\}
\end{equation}
It can be rewritten in terms of two-point correlation functions according to Wick's theorem \cite{Negele1988}
% \zc{check hypher usage}
\begin{equation}\label{eq:BIF}
\mathcal{L}_b^{(k)}\left(\tau_1, \ldots, \tau_M\right)= \begin{cases}0, & \text { if } M \text { is odd } \\ \sum_{\mathfrak{q} \in \mathcal{Q}_M} \prod_{\left(i, j\right) \in \mathfrak{q}} B^{(k)}(\tau_i,\tau_j), & \text { if } M \text { is even }\end{cases}
\end{equation}
Here $B^{(k)}$ is the two-point correlation function to be specified later in our test cases, and the set $\mathcal{Q}_M$ contains all possible pairings of integers $\{1,2,\cdots, M\}$. 
The two-point correlation function in this work is different but related to the two-point correlation in the previous research \cite{cai2020inchworm,cai2022fast,cai2023bold,wang2023real}.
The source of the difference comes from the location of the initial density in the Dyson expansion.
We will further elaborate on their relation later in the appendix.
% \begin{remark}
% \label{rmk_tpc}
%     We further clarify the expression of $B^{(k)}(\tau_i,\tau_j)$ here. In fact, 
%     \begin{equation}
%         B^{(k)}(\tau_i,\tau_j)=\operatorname{tr}_b\left\{\mathcal{T}\left[W_{b,I}(\tau_i)W_{b,I}(\tau_j)\rho_b^{(k)}(0)\right]\right\}
%     \end{equation}
%     is the complex conjugate of the two-point correlation function in our previous work\cite{wang2023real},
%     \begin{equation}
%         B^{(k)}(\tau_i,\tau_j)=\overline{\hat{B}^{(k)}(\tau_i,\tau_j)}
%     \end{equation}
%     where
%     \begin{equation}
%          \hat{B}^{(k)}(\tau_i,\tau_j)=\operatorname{tr}_b\left\{\mathcal{T}\left[\hat{W}_{b,I}(\tau_i)\hat{W}_{b,I}(\tau_j)\rho_b^{(k)}(0)\right]\right\},\quad \hat{W}_{b,I}(\tau)=e^{-\ii H_b|\tau|}W_b e^{\ii H_b |\tau|}
%     \end{equation}
%     The detailed proof is provided in \cref{apx_tpc}.
% \end{remark}

Our objective is to evaluate (\ref{eq:rhos_dyson}), which can be solved by employing the integro-differential equation developed by Wang and Cai \cite{wang2023real}.


% \yx{insert here}
% \ki{Please avoid using $\mathscr{U}$ since JCTC does not have this notation. You may refer to the final version of \cite{wang2023real} for the notations. I suggest to use $\Xi$ to replace $\mathscr{U}$.}
We first generalize the definition of $\mathcal{U}_0^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_k, \boldsymbol{\tau})$ to $\Xi_0^{(k)}(s_\ii, \boldsymbol{s},\boldsymbol{\alpha}_k, \boldsymbol{\tau},s_\ff)$ for $s_\ii <s_\ff$:
% \ki{We should not have $O_s$ in the following equation.}
% \zc{say more words on the purpose of inluding $s_\ii$ and $s_\ff$ in the expression.}
\begin{equation}\label{eq_U_generalized}
    \Xi_0^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s_\ff)
    =\begin{cases}
        \mathcal{T}[V_{s,I,\alpha_k^{(1)}}^{(k)}(s_1) \dots V_{s,I,\alpha_k^{(N)}}^{(k)}(s_N) W_{s,I}^{(k)}(\tau_1) \dots W_{s,I}^{(k)}(\tau_M) \rho_s^{(k)}(0)],
        &\text{~if~} 0\in[s_\ii,s_\ff], \\
        \mathcal{T}[V_{s,I,\alpha_k^{(1)}}^{(k)}(s_1) \dots V_{s,I,\alpha_k^{(N)}}^{(k)}(s_N) W_{s,I}^{(k)}(\tau_1) \dots W_{s,I}^{(k)}(\tau_M)],
        &\text{~if~} 0\notin[s_\ii,s_\ff].
    \end{cases}
\end{equation}
This generalization allows the derivation of integro-differential equation and the application of the inchworm algorithm. 

% For $s_\ii \leq\boldsymbol{s},\boldsymbol{\tau}\leq s_\ff$,
% \begin{equation}
%     \Xi_0^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s_\ff) = \Xi_0^{(k)}(s^1,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s_\ff)\Xi_0^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s^1)
% \end{equation}

$\rho^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_k)$ is redefined as $\Phi^{(k)}(\boldsymbol{s},\boldsymbol{\alpha}_k)$ in same way:
\begin{equation}\label{eq_rho_single_spin_generalized}
        \begin{split}
    \Phi^{(k)}\left(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,s_\ff\right)
    = &\left(\prod_{n=1}^{N} \sqrt{-\ii\,\sgn(s_{n})} \right)\sum_{M=0}^{\infty} (-\mathrm{i})^M \int_{s_\ii \leqslant \boldsymbol{\tau} \leqslant s_\ff}\left(\prod_{m=1}^M \operatorname{sgn}\left(\tau_m\right)\right) \\
    & \times \Xi_0^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_{k},\boldsymbol{\tau},s_\ff) \mathcal{L}_b^{(k)}(\boldsymbol{\tau}) \mathrm{d} \boldsymbol{\tau}
    \end{split}
\end{equation}
For any $s_\ii <s^1< s_\ff$ dividing the sequences $\boldsymbol{s}$, $\boldsymbol{\tau}$ into subsequences, $\Xi_0^{(k)}(s_\ff,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s_\ff)$ can be divided into two smaller quantities,
\begin{equation}
    \Xi_0^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s_\ff) = \Xi_0^{(k)}(s^1,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s_\ff)\Xi_0^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s^1)
\end{equation}

\zc{Therefore, the concatenation of two $\Phi$s will become part of another $\Phi$}

Under the specified initial condition:
 \begin{itemize}
    \item if $s_\ii \neq 0$,
    \begin{equation}\label{init1}
        \Phi^{(k)}(s_\ii, s_\ff = s_\ii) = \id^{(k)}
    \end{equation}
    \item if $s_N \neq 0$,
    \begin{equation}\label{init2}
        \begin{split}
&\qquad \Phi^{(k)}\left(s_\ii, \left(s_1, \cdots, s_N\right),\left(\alpha_k^{(1)},\ldots,\alpha_k^{(N)}\right), s_\ff = s_N\right)\\
&= \sqrt{-\ii\, \sgn(s_N)} V_{s,I,\alpha_k^{(N)}}^{(k)}(s_N) \Phi^{(k)}\left(s_\ii, \left(s_1,\cdots,s_{N-1}\right),\left(\alpha_k^{(1)},\ldots,\alpha_k^{(N-1)}\right), s_\ff = s_N\right).
\end{split}
    \end{equation}
\end{itemize}
It can be proven that the propagator $ \Phi^{(k)}\left(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,s_\ff\right)$, as outlined in \cref{eq_rho_single_spin_generalized}, satisfies the following integro-differential equation \cite{wang2023real}:
\begin{equation}
    \label{inchworm_differential_equation}
    \pdv{\Phi^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,s_\ff)}{s_\ff}
    = \mathcal{K}^{(k)}(s_\ii,\bs,\boldsymbol{\alpha}_k,s_\ff),
\end{equation}
where
\begin{equation}
\label{eq_K}
\begin{split}
    \mathcal{K}^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,s_\ff) = & \sum_{\substack{M=1\\M\text{~is~odd}}}^{\infty} (-\ii)^{M+1}
    \int_{s_\ii \leqslant \tau_1 \leqslant \dots \leqslant \tau_{M} \leqslant s_\ff} 
    \dd \tau_1 \dots \dd \tau_M
    \left( \prod_{m=1}^{M+1}  \, \sgn (\tau_m) \right)\\
    &\times W_s^{(k)}(s_\ff)
    \Xi^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s_\ff) \mathcal{L}_b^{c(k)}(\boldsymbol{\tau}),
\end{split}
\end{equation}
where $\boldsymbol{\tau}=\left(\tau_1,\ldots,\tau_M,\tau_{M+1}=s_\ff \right)$ is increasing and $\boldsymbol{s}=\left(\boldsymbol{s}_0,\ldots,\boldsymbol{s}_M\right)$ is chosen such that their extended sequence $\left(s_\ii,\boldsymbol{s}_0,\tau_1,\boldsymbol{s}_1,\tau_2,\ldots,\tau_{M-1},\boldsymbol{s}_M,\tau_M\right)$ is increasing. The system-associated operator $\Xi^{(k)}$ and bath influence functional are defined as:
\begin{equation}
\label{eq_xi}
    \begin{split}
        \qquad\Xi^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,\boldsymbol{\tau},s_\ff)=&\Phi^{(k)}(\tau_M,s_M,\alpha_k^{(M)},s_\ff)W_s^{(k)}(\tau_M)\Phi^{(k)}(\tau_{M-1},s_{M-1},\alpha_k^{(M-1)},\tau_M)\\
        &W_s^{(k)}(\tau_{M-1})\cdots W_s^{(k)}(\tau_{1})\Phi^{(k)}(s_\ii,s_0,\alpha_k^{(0)},\tau_1)
    \end{split}
\end{equation}

\begin{equation}
    \label{eq_L}
    \mathcal{L}_b^{c(k)}(\tau_1,\dots,\tau_{M+1})
    = \sum_{\mathfrak{q}\in\mathcal{Q}_{M+1}^c}
    \prod_{(j,{j'})\in\mathfrak{q}}
    B(\tau_j,\tau_{j'})
\end{equation}
where $\mathcal{Q}_{M+1}^c$ is the subset of $\mathcal{Q}_{M+1}$ consisting of pairs that are ``linked''\cite{cai2020inchworm,wang2023real}.


% \zc{Expand the following paragraph with some discussions on the computational cost}
This method offers a computationally efficient framework for evaluating the density matrices. While the intricate computational details are beyond the scope of this text, the reader may refer to the referenced work for an in-depth explanation.
The only difference between our work and previous work \cite{wang2023real} is that we may have more than one type of interaction operators, \emph{i.e.}, different colors of crosses.
% \ki{add some explanation of $\bar{M}$ here.}
%============== 
The differential-integro equation \cref{inchworm_differential_equation} reveals that the computation of $\Phi$s with longer time sequences depends on the knowledge of the ones with shorter sequences. Taking a uniform time step $\Delta t$ for simplicity, the time points $s_n$ and $\tau_m$ are multiple of $\Delta t$. Suppose the simulation of $\rho_I(t)$ is up to $t = \Delta t,\ldots, L\Delta t$ for a given positive integer $L$, and assume that all the diagrams of length less than $l\Delta t$ are already computed, then for the computational cost of evaluating $\Phi^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,s_\ii + l\Delta t)$ from $\mathcal{K}^{(k)}(s_\ii,\boldsymbol{s},\boldsymbol{\alpha}_k,s_\ii + (l-1)\Delta t)$ by forward Euler method is $\sum_{M=1,\text{ M odd}}^{\bar{M}}C_M \binom{M+l}{M}$, where $\bar{M}$ is the truncation parameter chosen in evaluating the series \cref{eq_rho_single_spin_generalized} and $C_M$ is the computational cost for computing each integrand which is assumed to be a constant since $\bar{M}\leq 5$ in our tests. The total number of different diagrams of length $l\Delta t$ $\leq$ $L\Delta t$ is 
 \begin{equation}
     \sum_{N=0}^{\bar{N}}(2L+1-l)\binom{N+l}{N}|A|^N\leq |A|^{\bar{N}}(2L+1-l)\binom{\bar{N}+l+1}{\bar{N}}
 \end{equation}
where $\bar{N}$ is the maximum number of couplings for each spin. The computational cost for the single-spin full propagators of all lengths is 
\begin{equation}
    \sum_{l=1}|A|^{\bar{N}}(2L+1-l)\binom{\bar{N}+l+1}{\bar{N}}\sum_{M=1,\text{ M odd}}^{\bar{M}}C_M\binom{\bar{M}+l}{\bar{M}}\lesssim |A|^{\bar{N}}L^{\bar{M}+\bar{N}+2}.
\end{equation}
In practise, $\bar{M}$, $\bar{N}$ and $|A|$ are relatively small. The computational cost scales as $O(L^{\bar{M}+\bar{N}+2})$.
% The computational cost becomes $O(KL^{\bar{M}+\bar{N}+2})$ if the $K$ spins have different parameters.
 
\section{Summation of propagators}
\label{sec_spin_connection}
In this section,
 we connect the single spin information to the full spin chain information by an iterative algorithm.
\begin{align}
% \label{eq_summation_propagators}
    &\mathbbm{p}^{[1]}(-t,\boldsymbol{s},\boldsymbol{\alpha}_1, t) = \rho_{s,I}^{(1)}(-t,\boldsymbol{s},\boldsymbol{\alpha}_1,t)\quad \text{for } \boldsymbol{\alpha}_1 \in A^{N} \label{eq_summation_propagators_1st_spin} \\
    &\mathbbm{p}^{[k+1]}(-t,\boldsymbol{s}, \boldsymbol{\alpha}_{k+1},t) = \sum_{N'=0}^\infty \sum_{\boldsymbol{\alpha'}_k \in A^{N'}} \int_{-t \leqslant \boldsymbol{s'}\leqslant t} \mathbbm{p}^{[k]}(-t, \boldsymbol{s'},\boldsymbol{\alpha'}_k,t) \nonumber \\
    &\qquad\qquad\qquad\qquad\qquad \otimes \rho_{s,I}^{(k+1)}(-t,[\boldsymbol{s'},\boldsymbol{s}],[\boldsymbol{\alpha}_k',\boldsymbol{\alpha}_{k+1}],t)\dd \boldsymbol{s'}, \nonumber \\
    &\qquad\qquad\qquad\qquad\qquad \text{for } k=1,\ldots,K-2 \text{ and for } \boldsymbol{\alpha}_{k+1} \in A^{N} \label{eq_summation_propagators_middle_spins}  \\
    &\mathbbm{p}^{[K]}(-t,t) = \sum_{N=0}^\infty \sum_{\boldsymbol{\alpha}_{K-1}\in A^N} \quad \int_{-t\leqslant \boldsymbol{s}\leqslant t}\mathbbm{p}^{[K-1]}(-t,\boldsymbol{s},\boldsymbol{\alpha}_{K-1}, t) \otimes \rho_{s,I}^{(K)}(-t,\boldsymbol{s},\boldsymbol{\alpha}_{K-1}, t)\dd \boldsymbol{s} \label{eq_summation_propagators_last_spin} 
\end{align}
In this context, $\boldsymbol{s}=\left(s_1,\ldots,s_N\right)$ and  $\boldsymbol{s'}=\left(s_1',\ldots,s_N'\right)$ are non-descending sequences. $\boldsymbol{\alpha}_{k+1}$ and $\boldsymbol{\alpha'}_k$ are sequences of corresponding coupling indices, where the $j$th component of $\boldsymbol{\alpha}_{k+1}$ is the index of the coupling operator acting on $(k+1)$th spin at time $s_j$. 
% $\mathcal{P}$ is a sorting operator that merges $\boldsymbol{s}$ and $\boldsymbol{s'}$ into a new non-descending list, as well as combines $\boldsymbol{\alpha'}_k$ and $\boldsymbol{\alpha}_{k+1}$.
$[\boldsymbol{s'},\boldsymbol{s}]$ and $[\boldsymbol{\alpha}_k',\boldsymbol{\alpha}_{k+1}]$ represent the merged ordered sequences.
% \ki{Do you think $\mathcal{P}(\boldsymbol{s'},\boldsymbol{s},\boldsymbol{\alpha}_k',\boldsymbol{\alpha}_{k+1})$ is a better choice?}
% \ki{Do we need subscriptions for $\boldsymbol{\alpha}$?}
% \zc{since we have \cref{eq_U_generalized} and the operators are ordered there, check if $\mathcal{P}$ for $\alpha$ can be removed.}

% \zc{move the following paragraph to the end of the section, after introducing the summation procedure and clarifying with examples.}

The computational process can be interpreted as iteratively concatenating with adjacent propagators, thereby extending the spin chain. Consider the concatenation of the 2nd spin, for $\boldsymbol{\alpha}_2 \in A^{N}$ and $|A|=3$,
\begin{equation}\label{eq:concate_2nd}
    \mathbbm{p}^{[2]}(-t,\boldsymbol{s},\boldsymbol{\alpha}_2, t)=\sum_{N'=0}^\infty \sum_{\boldsymbol{\alpha'}_1 \in A^{N'}}\int_{-t \leqslant \boldsymbol{s'}\leqslant t} \mathbbm{p}^{[1]}(-t,\boldsymbol{s'},\boldsymbol{\alpha'}_1, t)\otimes\rho_{s,I}^{(2)}(-t,[\boldsymbol{s},\boldsymbol{s'}],[\boldsymbol{\alpha'}_1,\boldsymbol{\alpha}_{2}],t)\dd \boldsymbol{s'},
\end{equation}

For the case of $\boldsymbol{s}=(s_1)$ and $\boldsymbol{\alpha}_{2}=(\alpha_{1}^{(1)})$, then we can express \cref{eq:concate_2nd} diagrammatically as:
\input{Path_Integral/concate_2nd}
Here, the open dashed line on the second spin indicates that it will be connected to the third spin in the subsequent iteration. The four diagrams in the second line represent the case where $N'=0$ and $N'=1$, while the third line, including $N'=2$, consists of $3^2$ diagrams to be summed. Similarly, for larger $N'$, there are $|A|^{N'}$ diagrams to be summed. We continue this concatenation process iteratively until we connect the last spin as $\cref{eq_summation_propagators_last_spin}$, 
\input{Path_Integral/concate_last_spin}

The process is similar to previous research \cite{wang2023real}, however, there are two main differences:
\begin{itemize}
    \item In the previous research \cite{wang2023real}, a specific observable is computed, and taking a trace is therefore required.
    In particular, taking the trace over the full spin chain can be separated into the traces of each spin.
    In this research, however, we use a propagator for each spin so that multiplications become tensor products in our work.
    % \zc{to be elaborated: we calculated the observable before and therefore taking trace is required.}
    The change, although it brings extra computational and memory cost, 
    allows further application of the transfer tensor method (TTM), 
    which will be introduced in \cref{sec_TTM}.
    \item In addition to the match of time sequences $\boldsymbol{s}$, the types of couplings $\boldsymbol{\alpha}$ should also be matched and summed due to the off-diagonal coupling.
    In particular, when $\vert A \vert = 1$, \emph{i.e.}, the diagonal coupling case, the indices $\boldsymbol{\alpha}$ will automatically match each other.
\end{itemize}

\begin{remark}
\label{rmk_connect_general_model}
    As discussed in \cref{rmk_general_model}, we consider the most general inter-spin couplings. In prevalent spin-$\frac{1}{2}$ chain models, such as the Heisenberg and the Frenkel-Exciton models, the interactions typically take the form of $\sigma_{\alpha}^{(k)} \otimes\sigma_{\alpha}^{(k+1)}$, as depicted in \cref{diagram_model_3terms}. Consequently, it is unnecessary to account for nine different colors of “crosses” for each spin, as only three types of interactions occur.
    However, our framework allows for the connection of differently colored crosses during summation steps. Specifically, the $V_I(s_n)$ in \cref{op:v_i} should be included with another subscript $\beta_{k+1}$ to reflect the couplings with the preceding spin, 
    \begin{equation*}
        V_I(s_n)=\sum_{k=1}^{K-1}\sum_{\alpha_k\in A}\sum_{\beta_{k+1}\in A}V_{I,\alpha_k}^{(k)}(s_n)\otimes V_{I,\beta_{k+1}}^{(k+1)}(s_n)
    \end{equation*}
    Similarly, the single propagators $\rho^{(k)}(\boldsymbol{s}',\boldsymbol{\alpha}_k')$ in \cref{eq_rho_k} are extended to $\rho^{(k)}(\boldsymbol{s}',\boldsymbol{\alpha}_k',\boldsymbol{\beta}_k')$. 
    The concatenation process in \cref{eq_summation_propagators_middle_spins} should be modified accordingly, another summation over $\boldsymbol{\beta}_{k+1}'$ is required, and $ \mathbbm{p}^{[k]}(-t, \boldsymbol{s'},\boldsymbol{\alpha'}_k,t)$ should be tensor-product with $\rho_{s,I}^{(k+1)}(-t,$ $[\boldsymbol{s'},\boldsymbol{s}],$ $[\boldsymbol{\alpha}_k',\boldsymbol{\alpha}_{k+1}],$ $[\boldsymbol{\beta}_{k+1}'],t)$. This ensures that the coupling $\sigma_{\alpha_k}^{(k)} \otimes \sigma_{\beta_{k+1}}^{(k+1)}$ along sequence $\boldsymbol{s}'$ is matched between the $k$th and the $(k+1)$th spin.
    This adaptation allows our approach to be applied to general coupling cases.
\end{remark}

% \begin{remark}
% \label{rmk_connect_general_model}
%     In \cref{rmk_general_model}, we mention the most general inter-spin couplings.
%     In this model\zc{to be elaborated}, we do not need to consider 9 different colors of ``crosses'' on each spin since there are only three types of interactions.
%     Therefore, considering three types of interactions is more than enough.\zc{unclear}
%     However, in this case, different colors of crosses can also be connected in the summation steps.
%     So our idea can be extended to the general coupling case.
%     \zc{similar as remark 1, say more words on matching crosses in general condition}
% \end{remark}

The computational cost of propagators $\rho_{s,I}^{(k)}(-t,\boldsymbol{s},\boldsymbol{\alpha}_k,t)$ has been estimated as $O(|A|^{\bar{N}}L^{\bar{N}+\bar{M}+2})$, as discussed at the end of \Cref{sec_diagrammatic_representation}. We now evaluate the computational cost for calculating all possible $\mathbbm{p}^{[k+1]}(-t,\boldsymbol{s},\boldsymbol{\alpha}_{k+1},t)$ at time $t=l\Delta t$ for sequences $\boldsymbol{s}$ of length at most $\bar{N}$. This is based on the already computed $\rho_{s,I}^{(k+1)}(-t,[\boldsymbol{s}',\boldsymbol{s}],[\boldsymbol{\alpha}_k',\boldsymbol{\alpha}_{k+1}],t)$ for $N'\leq \bar{N}-N$, as outlined in \cref{eq_summation_propagators_middle_spins},
\begin{equation}
\quad\sum_{N=0}^{\bar{N}}\binom{2l+N}{N}|A|^{N}\sum_{N'=0}^{\bar{N}-N}\binom{2l+N'}{N'}|A|^{N'}\lesssim  \bar{N}|A|^{\bar{N}}l^{\bar{N}}
\end{equation}
% Consequently, the cost to compute $\mathbbm{p}^{[K]}(-t,t)$, which approximates $\rho_{s,I}(t)$ up to $t=L\Delta t$, is $O(|A|^{\bar{N}}L^{\bar{N}+1})$. 
% Given that $|A|$ is typically small, the overall computational cost of our simulation up to $L$ time steps is therefore $O(L^{\bar{N}+\bar{M}+2})$.
Given that $|A|$ is typically small, the overall computational cost of our simulation up to $L$ time steps is therefore $O(L^{\bar{N}+\bar{M}+2})$.

% \begin{remark}
% \label{rmk_connect_general_model}
%     In \cref{rmk_general_model}, we mention the most general inter-spin couplings.
%     It is this model\zc{to be elaborated}, we do not need to consider 9 different colors of ``crosses'' on each spin since there are only three types of interactions.
%     Therefore, considering three types of interactions is more than enough.\zc{unclear}
%     However, in this case, different colors of crosses can also be connected in the resummation steps.
%     So our idea can be extended to the general coupling case.
%     \zc{similar as remark 1, say more words on matching crosses in general condition}
% \end{remark}

% \zc{Comparison with MPI: our advantage is using fewer crosses and saving cost; MPI's advantage is their fast computation in off-diagonal models.}
\begin{remark}
    \label{rmk_computation_cost}
    We would like to comment on the difference in the computational cost of our method with our previous work on diagonal coupling cases. The only increase is the cost of matching the ``crosses'' with different colors. For diagonal coupling cases $|A|=1$, the total computational cost scales as $O(L^{\bar{M}+\bar{N}+2})$. In our experiments, $|A|$ is at most 3, while the presence of $|A|$ increases the computational cost, it does so without altering the polynomial scaling with $L$, as the primary complexity still scales with $L^{\bar{M}+\bar{N}+2}$, maintaining a similar order of magnitude.
    We also compare the computational cost of our method and that of the Factorized MPI methodology. The procedure involves sequential matrix-vector multiplications and evaluates the path sum separately. For diagonal coupling, the number of operations per unit is $(4L+5)2^{2L+2}$; for the non-diagonal case, where the linking of non-terminal units is predominant, which needs $4(L+4)2^{2L+4}$ per unit\cite{kundu2021efficient}. Such costs scale exponentially as the number of time steps increases. Our method mitigates this exponential increase by employing truncation in path integrals and limiting computations to paths where the number of inter-spin interactions does not exceed $\bar{N}$. However, our approach relies on the tensor-product decomposition of non-diagonal couplings. As the number of decompositions, denoted by $|A|$, increases, so does the computational cost. Unlike our method, the computational cost of the MPI does not change with different types of non-diagonal couplings. 
\end{remark}

% We further clarify the mathematical meaning of these diagrams,

% \begin{tikzpicture}[baseline=0]
%             \filldraw[fill=lightgray] (-1,0.55-0.4) rectangle (1,0.65-0.4);
%             \filldraw[fill=lightgray] (-1,0.15-0.4) rectangle (1,0.25-0.4);
%             % \draw[black, line width=1pt] (-1,0.6-0.4) -- (-1,0.2-0.4);
%             % \draw[black] (+1,0.6-0.4) -- (+1,0.2-0.4);
%             \node[text=applegreen] at (-0.5,0.2-0.4) {$\times$};
%             % \node[text=red] at (-0.5,-0.2-0.4) {$\times$};
%             \draw[black, densely dotted, line width = 1pt] (-0.5,0.2-0.4) -- (-0.5,-0.2-0.4);
%             \node[text=blue] at (0.2,0.6-0.4) {$\times$};
%             \node[text=blue] at (0.2,0.2-0.4) {$\times$};
%             \draw[black, densely dotted, line width = 1pt] (0.2,0.6-0.4) -- (0.2,0.2-0.4);
% \end{tikzpicture}
% the corresponding propagators are $\rho^{(1)}(-t,s_1,\alpha_2^{(1)},t)$, $\rho^{(2)}(-t,(s_1,s_2),(\alpha_1^{(1)},\alpha_2^{(2)}),t)$ \ki{What is $s_1,s_2$ here?}\yx{maybe we can omit this clarification here?} \\

% \begin{tikzpicture}[baseline=0]
%         \filldraw[fill=lightgray] (-1,0.55-0.4) rectangle (1,0.65-0.4);
%         \filldraw[fill=lightgray] (-1,0.15-0.4) rectangle (1,0.25-0.4);
%         % \draw[black, line width=1pt] (-1,0.6-0.4) -- (-1,0.2-0.4);
%         % \draw[black] (+1,0.6-0.4) -- (+1,0.2-0.4);
%         \node[text=red] at (-0.5,0.2-0.4) {$\times$};
%         % \node[text=red] at (-0.5,-0.2-0.4) {$\times$};
%         \draw[black, densely dotted, line width = 1pt] (-0.5,0.2-0.4) -- (-0.5,-0.2-0.4);
%         \node[text=yellow] at (0.1,0.6-0.4) {$\times$};
%         \node[text=yellow] at (0.1,0.2-0.4) {$\times$};
%         \draw[black, densely dotted, line width = 1pt] (0.1,0.6-0.4) -- (0.1,0.2-0.4);
%         \node[text=red] at (-0.8,0.6-0.4) {$\times$};
%         \node[text=red] at (-0.8,0.2-0.4) {$\times$};
%         \draw[black, densely dotted, line width = 1pt] (-0.8,0.6-0.4) -- (-0.8,0.2-0.4);
%         \end{tikzpicture}
% the corresponding propagators are $\rho(-t,(s_2,s_1),(\alertyellow{2},\alertred{0}),t)$, $\rho(-t,(s_3,s_2,s_1),(\alertyellow{2},\alertred{0},\alertred{0}),t)$

% \input{achemso/Path_Integral/diagram_equation}



==> diagram_model.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=1]
% Yellow nodes (spins)
\filldraw[fill=yellow] (0,0) circle (1cm);
\node[text=black] at (0,0) {$H_s^{(1)}$};
\filldraw[fill=yellow] (4,0) circle (1cm);
\node[text=black] at (4,0) {$H_s^{(2)}$};
\filldraw[fill=yellow] (8,0) circle (1cm);
\node[text=black] at (8,0) {$H_s^{(3)}$};
\filldraw[fill=yellow] (12,0) circle (1cm);
\node[text=black] at (12,0) {$H_s^{(4)}$};

% Green nodes (harmonic baths)
\filldraw[fill=green] (0,-4) circle (1cm);
\node[text=black] at (0,-4) {$H_b^{(1)}$};
\filldraw[fill=green] (4,-4) circle (1cm);
\node[text=black] at (4,-4) {$H_b^{(2)}$};
\filldraw[fill=green] (8,-4) circle (1cm);
\node[text=black] at (8,-4) {$H_b^{(3)}$};
\filldraw[fill=green] (12,-4) circle (1cm);
\node[text=black] at (12,-4) {$H_b^{(4)}$};

% Dashed lines between yellow and green nodes
\draw[dashed] (0,-1) -- (0,-3);
\node[text=black] at (0,-2) {$W_s^{(1)}\otimes W_b^{(1)}$};
\draw[dashed] (4,-1) -- (4,-3);
\node[text=black] at (4,-2) {$W_s^{(2)}\otimes W_b^{(2)}$};
\draw[dashed] (8,-1) -- (8,-3);
\node[text=black] at (8,-2) {$W_s^{(3)}\otimes W_b^{(3)}$};
\draw[dashed] (12,-1) -- (12,-3);
\node[text=black] at (12,-2) {$W_s^{(4)}\otimes W_b^{(4)}$};

% Solid lines between yellow nodes
% Adjust the vertical shift (the 0.25*\y term) to increase the spacing
\draw[color=red] (1,0.2) -- (3,0.2);
\draw[color=blue] (1,0) -- (3,0);
\draw[color=amethyst] (1,-0.2) -- (3,-0.2);
\node[text=black] at (2,0.6) {$V^{(1,2)}$};

\draw[color=red] (5,0.2) -- (7,0.2);
\draw[color=blue] (5,0) -- (7,0);
\draw[color=amethyst] (5,-0.2) -- (7,-0.2);
\node[text=black] at (6,0.6) {$V^{(2,3)}$};

\draw[color=red] (9,0.2) -- (11,0.2);
\draw[color=blue] (9,0) -- (11,0);
\draw[color=amethyst] (9,-0.2) -- (11,-0.2);
\node[text=black] at (10,0.6) {$V^{(3,4)}$};
\end{tikzpicture}

\caption{
Illustration of a chain with four spins where each spin is coupled with a harmonic bath. Each yellow circle stands for a spin and each green circle stands for a harmonic bath.
The solid lines with different colors between two spins indicate the coupling between two spins
and a dashed line stands for the coupling between a spin and its bath.
% Illustration of the Heisenberg chain with four spins where each spin is coupled with a harmonic bath. Each yellow circle stands for a spin and each green circle stands for a harmonic bath. The solid lines with different colors between two spins indicate the coupling given by $\sigma_x\otimes\sigma_x$,$\sigma_y\otimes\sigma_y$ and $\sigma_z\otimes\sigma_z$; a dashed line between a yellow circle and a green circle stands for the coupling relation between a spin and its bath.
}
\label{diagram_model}
\end{figure}
